The View Update Problem Revisited

In this paper, we revisit the view update problem in a relational setting and propose a framework based on the notion of determinacy under constraints. Within such a framework, we characterise when a view mapping is invertible, establishing that this is the case precisely when each database symbol has an exact rewriting in terms of the view symbols under the given constraints, and we provide a general effective criterion to understand whether the changes introduced by a view update can be propagated to the underlying database relations in a unique and unambiguous way. Afterwards, we show how determinacy under constraints can be checked, and rewritings effectively found, in three different relevant scenarios in the absence of view constraints. First, we settle the long-standing open issue of how to solve the view update problem in a multi-relational database with views that are projections of joins of relations, and we do so in a more general setting where views are defined by arbitrary conjunctive queries and database constraints are stratified embedded dependencies. Next, we study a setting based on horizontal decompositions of a single database relation, where views are defined by selections on possibly interpreted attributes (e.g., arithmetic comparisons) in the presence of domain constraints over the database schema. Lastly, we look into another multi-relational database setting, where views are defined in an expressive "Type" Relational Algebra based on the n-ary Description Logic DLR and database constraints are inclusions of expressions in that algebra.

==> related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\noindent %
As already mentioned, the understanding of the theoretical foundations of the
view update problem is due to the seminal work of Bancilhon and Spyratos
\cite{BanSpy:1981:usr}. %
In addition to the notions of translation and translatability, that we revisited
in Section~\ref{sec:framework}, they also introduce the notions of \emph{view
  complement} and \emph{translation under constant complement}. %
Given a view that is lossy (i.e., does not preserve all of the informative
content of the underlying database) a view complement is a second view that
contains enough information to attain losslessness when combined with the
original view. %
The constant complement principle prescribes that updates on the view must not
influence, directly or indirectly, the content of the view complement. %
In this paper, we did not discuss the issues concerning these notions, but it
suffices to say that the results of Section~\ref{sec:framework} about the
invertibility of views and the translatability of view updates hold also in the
presence of view complements \cite{FraGua:2012:TR}.

Cosmadakis and Papadimitriou \cite{CosPap:1984:urv} study a restricted setting
that consists of only two view symbols defined by projections over a
uni-relational database schema. %
They show that, in the absence of view constraints, when the database
constraints are functional and join dependencies, the view is invertible if and
only if the database symbol can be rewritten as the join of the two view
symbols. %
Their result has been generalised in \cite{FraGua:2012:tvu} to an arbitrary
number of view symbols defined by acyclic projections and database constraints
consisting of full dependencies. %
Both \cite{FraGua:2012:tvu} and \cite{CosPap:1984:urv} are special cases of the
setting discussed in Section~\ref{sec:cq-views}, where the rewriting is a priori
known to be the join, and determinacy under constraints is finitely controllable
(i.e., it holds or not independently on whether infinite instances are
allowed). %
To the best of our knowledge, \cite{CosPap:1984:urv} is the only comprehensive
work in which the abstract framework by Bancilhon and Spyratos is applied to a
relational setting. %
Necessary and sufficient conditions are provided for the translatability of
insertions, deletions and replacements w.r.t.\ an instance, when the database
constraints are fd's. %
Our general criterion subsumes all these conditions, it applies for more
expressive database constraints (namely, stratified embedded dependencies), can
be checked locally on the view schema, and allows for more general classes of
updates (e.g., conditional and transactional) rather than single insertions,
deletions and replacements. %
In addition, the problem of checking translatability of view updates w.r.t.\
\emph{every} view state is not addressed in \cite{CosPap:1984:urv}, while our
Theorem~\ref{thm:fol-translat} provides a characterisation of translatability
w.r.t.\ every view state in terms of logical implication. %
An example of a view update that is translatable in this sense is given in
Example~\ref{exa:toy-example-2}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                         % Determinacy and rewriting %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Nash et al.\ \cite{NaSeVi:2010:vqd} investigate the related problem of deciding
whether the answer to a query $q$ over a database schema $\R$ is determined by a
set of view symbols $\V$ defined over $\R$. %
For view definitions and queries expressed in languages ranging from FOL to
\cqs, they systematically study whether determinacy is decidable and whether the
query language is \emph{complete} for rewritings, meaning that queries
determined by views can be rewritten in terms of the view symbols by using the
same language in which they are originally expressed. %
The notion of determinacy used in \cite{NaSeVi:2010:vqd} differs from the one in
this article in that we consider it w.r.t.\ a set of global constraints that,
along with the view definitions, include also additional constraints over the
database and the view schemas. %
Moreover, we are only interested in atomic queries, and rewritings that are
general domain-independent function-free FOL formulae, rather than belonging to
the same fragment in which queries are expressed. %
We remark that our result about determinacy of Section~\ref{sec:cq-views} is not
contradicted by the fact that the class \cq\ of conjunctive queries is not
complete for \cq-to-\cq\ rewritings \cite{NaSeVi:2010:vqd}. %
Rather, in the absence of database constraints (i.e., $\Sigma_\R = \emptyset$),
a corollary of Theorem~\ref{thm:cqrw-main} is that \cq\ is complete for
AQ-to-\cq\ rewritings, where AQ denotes the class of atomic queries.

Fan et al.\ \cite{FaFlLi:2012:vdp} study the connection between determinacy and
invertibility of views w.r.t.\ a query. %
The setting is similar to that of \cite{NaSeVi:2010:vqd}, where the global
constraints $\Sigma$ are given by exact view definitions only, and there are no
constraints on either the database schema $\R$ nor the view schema $\V$. %
Recasting the definition in \cite{FaFlLi:2012:vdp} to match our notation and
terminology, the view $f$ induced by $\Sigma$ is said to be \emph{invertible
  relative to} a query $q$ over $\R$ if there exists a query $q^{-1}$ such that
$q({I_{\R}}) = q^{-1}\big( f(I_{\R}) \big)$ for every database instance
$I_{\R}$. %
Intuitively, this means that $f$ (called a \emph{transformation} in
\cite{FaFlLi:2012:vdp}) preserves, without any loss, the information selected by
the query $q$. %
This is closely related to our notion of invertibility of a view: the view $f$
is invertible (in our sense) iff it is invertible relative to every atomic query
over $\R$, that is, relative to $q(\overline{x}) = R(\overline{x})$, for each $R
\in \R$. %
In other words, $f$ is lossless (i.e., invertible) when it preserves the
information contained in each database relation, selected by the (atomic) query
over the corresponding database symbol. %
In light of the strong connection between these two notions of invertibility,
and between our notion of determinacy under constraints and determinacy in
\cite{NaSeVi:2010:vqd}, as we show that invertibility of views coincides with
determinacy under constraints, in \cite{FaFlLi:2012:vdp} it is shown that
invertibility relative to a query coincides with determinacy in the sense of
\cite{NaSeVi:2010:vqd}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
                               % Data Exchange %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The framework we presented in Section~\ref{sec:framework} is reminiscent of a
Data Exchange (DE) \cite{FKMP2003:des} setting. %
In DE the connection between source and target schemas is commonly expressed by
means of so-called \emph{source-to-target} tgd's (s-t tgd's), that is, tgd's
where the l.h.s.\ of the implication mentions only source symbols while the
r.h.s.\ mentions only target symbols. %
A \emph{schema mapping} in DE is a triple $\tuple{\sign{S},\sign{T},\Gamma}$,
where $\sign{S}$ is the source schema, $\sign{T}$ is the target schema and
$\Gamma$ is a set of s-t tgd's over $\sign{S} \cup \sign{T}$. %
A schema mapping in this sense is not a view mapping in our sense, but it rather
represents a class of them, namely that of all the views under $\Gamma$,
according to Definition~\ref{def:view-under-constr}. %
Indeed, for a given source instance $I_{\sign{S}}$, in general there can be more
than one target instance $I_{\sign{T}}$ such that their disjoint union
$\umod{I_{\sign{S}}}{I_{\sign{T}}}$ (see Section~\ref{sec:preliminaries}) is a
model of $\Gamma$, therefore $\sign{S} \ndtm_\Gamma \sign{T}$. %
On the contrary, by considering exact view definitions, we ensure a one-to-one
correspondence between views and sets of global constraints inducing them (up to
logical equivalence). %
Clearly, also the notion of inverse of a schema mapping in DE differs from the
standard notion of inverse function in the mathematical sense (and ours). %
Indeed, no schema mapping in DE has a unique inverse, although under certain
circumstances there is, among the others, only one inverse with a specific
form~\cite{FagNas:2010:sis}. %
The case in which there is a unique target instance for a given source instance
under the schema mapping, namely when schema mappings can be transformed into
proper view mappings via an abduction process, is analysed in
\cite{FrNgSh:2012:dap}.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

